A Non-Asymptotic Framework for Approximate Message Passing in Spiked Models

Approximate message passing (AMP) emerges as an effective iterative paradigm for solving high-dimensional statistical problems. However, prior AMP theory -- which focused mostly on high-dimensional asymptotics -- fell short of predicting the AMP dynamics when the number of iterations surpasses $o\big(\frac{\log n}{\log\log n}\big)$ (with $n$ the problem dimension). To address this inadequacy, this paper develops a non-asymptotic framework for understanding AMP in spiked matrix estimation. Built upon new decomposition of AMP updates and controllable residual terms, we lay out an analysis recipe to characterize the finite-sample behavior of AMP in the presence of an independent initialization, which is further generalized to allow for spectral initialization. As two concrete consequences of the proposed analysis recipe: (i) when solving $\mathbb{Z}_2$ synchronization, we predict the behavior of spectrally initialized AMP for up to $O\big(\frac{n}{\mathrm{poly}\log n}\big)$ iterations, showing that the algorithm succeeds without the need of a subsequent refinement stage (as conjectured recently by \citet{celentano2021local}); (ii) we characterize the non-asymptotic behavior of AMP in sparse PCA (in the spiked Wigner model) for a broad range of signal-to-noise ratio.

==> backup_initialization.tex <==
Note, however, that this procedure only outputs a vector of dimensional $|\mathcal{I}_{\widehat{j}}^c|$, 
and it remains to estimate the remaining entries of $\vstar$.  
To do so, we put forward a two-step AMP algorithm that returns $u_{t} \in \real^{n}$ for each $t$, 
built upon Algorithm~\ref{alg:split}. 
%
\begin{enumerate}
	\item[i)] 
Run Algorithm~\ref{alg:split} to obtain $x_{t} \in \real^{|\mathcal{I}_{\widehat{j}}^c|}$. 

\item[ii)] 
% Since $x_{t}$ is only supported on set $\mathcal{I}_{\widehat{j}}^c$, we shall estimate the values on the other coordinates as well. In order to do so, we 
Run Steps 1-3 of Algorithm~\ref{alg:split} again with the input matrix being $M_{\mathcal{I}_{\widehat{j}}^{c}, \mathcal{I}_{\widehat{j}}^{c}}$; 
		namely, we randomly sample $N$ subsets $\overline{\mathcal{I}}_{i} \subset \mathcal{I}_{\widehat{j}}^c$ ($i \in [N]$), 
		and select the best one $\overline{\mathcal{I}}_{\widehat{i}}$. 
%
%	while Step 1, 2 are executed on set $\mathcal{I}_{\widehat{j}}^c$ \footnote{Here, we replace set $[n]$ in Step 1 with set $\mathcal{I}_{\widehat{j}}^c$} by 
%generating index sets $\overline{\mathcal{I}}_{i} \subset \mathcal{I}_{\widehat{j}}^c$ for $i \in [N]$, 
%and selecting the best $\overline{\mathcal{I}}_{\widehat{i}}$.
%
Clearly, one has $[n] = {\mathcal{I}}_{\widehat{j}}^c \cup \overline{\mathcal{I}}_{\widehat{i}}^{c}$. 

\item[iii)] Run AMP \eqref{eqn:AMP-updates-sparse} on the submatrix $M_{\overline{\mathcal{I}}_{\widehat{i}}^c, \overline{\mathcal{I}}_{\widehat{i}}^c}$
to obtain $\overline{x}_{t} \in \real^{|\overline{\mathcal{I}}_{\widehat{i}}^c|}$.
%Now it is sufficient to combine the outputs of two AMP sequences with 
%$x_{t} \in \real^{|\overline{\mathcal{I}}_{\widehat{j}}^c|}$
%and 
%$\overline{x}_{t} \in \real^{|\overline{\mathcal{I}}_{\widehat{i}}^c|}$.

\item[iv)] To merge $x_t$ and $\overline{x}_t$, 
	we set the final estimate $u \in \real^{n}$ as follows: 
\begin{equation}
\label{eqn:estimate-u}
\begin{aligned}
	u_t^{i} &= x_t^i, \qquad \text{for } i \in \mathcal{I}_{\widehat{j}}^c \\
	u_t^{i} &= \overline{x}_t^i, \qquad \text{for } i \in \mathcal{I}_{\widehat{j}}.
	% \mathsf{ST}_{\tau_t}\big(\overline{x}_t^i\big) + s_t^i, \qquad \text{for } i \in \mathcal{I}_{\widehat{j}},
\end{aligned}
\end{equation}
% where $s_t^i \stackrel{\mathrm{i.i.d.}}{\sim} \mathcal{N}(0, 1/n)$.
\end{enumerate}

\noindent 
We are ready to characterize the properties of the final estimate $u_{t}$ --- in a non-asymptotic sense --- as follows. 
%
\begin{cors}
\label{cor:sparse-init-2}
%
With probability at least $1 - O(n^{-10})$, the estimator \eqref{eqn:estimate-u} satisfies
%
\begin{subequations}
\label{eqn:finale-prop3}
\begin{align}
\label{eqn:decomp-1-sparse}
	u_{t}^i &= \alpha_{t} \vstar_{i} 
	+ \sum_{j = 1}^{t-1} \beta_{t-1}^j\phi_{j, i} 
	+ \xi_{t-1, i}, \qquad i \in \mathcal{I}^c_{\widehat{j}} \\
%
	u_{t}^i &= \overline{\alpha}_{t} \vstar_i + \sum_{j = 1}^{t-1} \overline{\beta}_{t-1}^j \overline{\phi}_{j, i} + \overline{\xi}_{t-1, i}, \qquad i \in \mathcal{I}_{\widehat{j}}
\end{align}
where 
\begin{align*}
	&\|\vstar_{\mathcal{I}_{\widehat{j}}^{c}}\|^2_2, ~\|\vstar_{\mathcal{I}_{\widehat{i}}^{c}}\|^2_2 = 1 - p + o(p), \\
	& \|\beta_{t-1}\|_2,~\|\overline{\beta}_{t-1}\|_2 = 1, \\
	&\alpha_{t},~\overline{\alpha}_t = \lambda\sqrt{1 - p + o(p)}  + O\Big(\sqrt{\frac{k + t\log^3 n}{n}}\Big),\\
	\text{and}\qquad &\ltwo{\xi}, ~\ltwo{\overline{\xi}} \lesssim \sqrt{\frac{(1 - p) (k+t\log^3 n)}{n}}, 
\end{align*}
where $p \asymp \frac{\log n}{k}$ and $\phi_j \stackrel{\text{i.i.d.}}{\sim} \mathcal{N}(0, \frac{1}{n} I_{|\mathcal{I}^c_{\widehat{j}}|})$ and $\overline{\phi}_j \stackrel{\text{i.i.d.}}{\sim} \mathcal{N}(0, \frac{1}{n} I_{|\mathcal{I}^c_{\widehat{i}}|})$. 
\end{subequations}
\end{cors}




\yuting{check the scaling here.}
% \begin{remark}
Corollary~\ref{cor:sparse-init-2} is a direct consequence of Theorem~\ref{thm:sparse} as the AMP algorithm in consideration --- albeit in slightly small scale --- starts with an informative and independent initialization point. Thus, we omit its proof here.  
We remind the readers that, while for each $j$, the corresponding initialization point $x^{j}$ is independent of $M_{\mathcal{I}_j^{c},\mathcal{I}_j^{c}}$, the algorithm selects the best $j$ as in expression~\eqref{eqn:sparse-choose-j}. 
To prove such data-dependent initialization is valid, similar to Corollary~\ref{cor:sparse-init-1}, we shall take a union bound over all possible choices of $j \in \mathcal{S}_{0}$ and similarly, choices of $i$ (both of which has $N$ choices). 
Corollary~\ref{cor:sparse-init-2} holds true if the corresponding decomposition holds simultaneously for all these $N^{2}$ AMP sequences, which happens with probability at least $1 - O(n^{-10})$ as ensured by Theorem~\ref{thm:sparse}.
% \end{remark}
By some direct algebra~(as in~\eqref{eqn:l2-error-hp}), an estimator based on $u_{t}$ yields $\ell_{2}$ loss of order $O\bigg(\sqrt{\frac{k\log n + t\log^3 n}{n\lambda^2}}\bigg)$. 





==> models.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Problem settings and background}
%\label{sec:models}

%
%As mentioned previously, each iterate of the AMP procedure can be characterized by a low-dimensional recursive formula termed the state evolution. 
%Specifically, consider the AMP algorithm~\eqref{eqn:AMP-updates} for the spiked Wigner model~\eqref{eqn:wigner}. 
%Assuming that the empirical distribution of $\{\sqrt{n} v_i^{\star}\}_{i=1}^{n}$ \footnote{Here, we adopt the scaling $\sqrt{n}$ to be consistent with this paper, since $\ltwo{\vstar} = 1$ in our assumption.} converges weakly to a probability distribution $\mu_{V}$ on $\mathbb{R}$ with unit second moment, \citet{montanari2021estimation} showed that the behavior of AMP can be characterized via the following system with two scalars 
%%
%\begin{subequations}
%\label{eq:SE-Montanari}
%\begin{align}
%	\alpha_{t+1} &= \lambda \myE\big[V \eta_t(\alpha_t V + \beta_t G)\big] \\
%	\beta_{t+1}^2 &= \myE\big[\eta_t^2(\alpha_t V + \beta_t G)\big],
%\end{align}
%\end{subequations}
%where ${V \sim \mu_{V}}$ and ${G\sim \mathcal{N}(0,1)}$ are independent random variables.
%In particular, given any pseudo Lipschitz test function $\Psi: \mathbb{R} \times \mathbb{R} \to \mathbb{R}$ obeying $|\Psi(x) - \Psi(y)|\leq C(1+\|x\|_{2} + \|y\|_{2})\cdot\|x - y\|_{2}$ for some universal constant $C > 0$, it holds almost surely that 
%\begin{align}
%	\lim_{n\to \infty} \frac{1}{n}\sum_{i=1}^n \Psi(\sqrt{n}v^\star_i, \sqrt{n} x^i_{t}) 
%	=
%	\myE \Big[\Psi(V, \alpha_tV + \beta_t G)\Big] .
%\end{align} 
%Here state evolution formula \eqref{eq:SE-Montanari} is derived respectively in \cite{fletcher2018iterative} for AMP initialized at an independent and informative point (which has positive non-vanishing correlation with $\vstar$), and in \citet{montanari2021estimation} when AMP is spectrally initialized. 
%In this paper, we show that the performances of AMP can be captured by a finite-sample version of the state evolution that agrees with \eqref{eq:SE-Montanari} in the large $n$ limit. 
%These characterizations are especially useful if one aims to understand the convergence rate or the optimization properties regarding the AMP iterates and its limiting point. 
%
%
%One nice feature of the state evolution is that it can be used to design proper denoising functions $\eta_{t}$ (see, \cite{bayati2011dynamics,montanari2021estimation}).  
%Recognizing that each coordinate of the AMP updates at step $t$ behaves like $\alpha_tV + \beta_t G$ where $G$ follows a standard normal distribution that is independent of $V$, $\eta_{t}$ serves as the function used to recover $V$ from noisy observation $\alpha_tV + \beta_t G$.
%Therefore, a natural choice of $\eta_t$ at time $t$ maximizes the ratio 
%$\Exs\big[V \eta_t(\alpha_t V + \beta_t G)\big]/\sqrt{\Exs\big[\eta_t^2(\alpha_t V + \beta_t G)\big]}$. When the distribution $\mu_{V}$ is known, the above principle leads to the choice
%\begin{align}
%\label{eqn:eta-principle}
%	\eta_t(x) \propto \Exs[V \mid \alpha_t V + \beta_t G = x],
%\end{align}
%up to some multiplying constant. 
%In Section~\ref{sec:examples}, we revisit two examples, (1) the $\mathbb{Z}_{2}$ synchronization where $\vstar_{i}$ takes the value $\{\pm\frac{1}{\sqrt{n}}\}$, both with probability $1/2$ and (2) the sparse recovery case, where $\vstar$ is assumed to have $k$ non-zero entries. 
%In both cases, $\eta_{t}$ is selected according to \eqref{eqn:eta-principle}, and 
%we shall elaborate more about the choices of $\eta_{t}$ when we get to these examples. 


















==> proof-sparse-prop3.tex <==

\subsection{Proof of Proposition~\ref{eqn:hard-regime-sparse}}
\label{sec:pf-decomp-2-stage}

Given every fixed $j \in \mathcal{S}_{0}$, consider the AMP initialized at $x^{j}$ (independent of $M_{\mathcal{I}^c_j, \mathcal{I}_j^c}$). 
Since $\langle v_{\mathcal{I}_{j}^{c}}^{\star}, x^j \rangle/\|v_{\mathcal{I}_{j}^{c}}^{\star}\|_2 \asymp 1$, Theorem~\ref{thm:sparse} justifies the decomposition for AMP iterates with corresponding error control in \eqref{eqn:soccer} holding with probability at least $1 - O(n^{-11}).$ 
Taking a union bound over all possible choices of $j \in \mathcal{S}_{0}$ (which in total has $N$ choices), the corresponding inequalities~\eqref{eqn:soccer} hold simultaneously with probability at least $1 - O(n^{-10}).$
Now since Proposition~\ref{prop:sparse-split} ensures that $\widehat{j} \in \mathcal{S}_{0}$ with probability at least $1 - O(n^{-10})$, we can conclude: 
with probability at least $1 - O(n^{-10})$, the execution of AMP on $M_{\mathcal{I}_{{j}}^c,\mathcal{I}_{{j}}^c}$ leads to decomposition  
\begin{subequations}
\label{eqn:finale-prop3}
\begin{align}
\label{eqn:decomp-1-sparse}
	x_{t}^\ell 
	= \alpha_{t} \vstar_{\ell} 
	+ \sum_{j = 1}^{t-1} \beta_{t-1}^j\phi_{j, \ell} 
	+ \xi_{t-1, \ell}, \qquad \ell \in \mathcal{I}^c_{\widehat{j}}
\end{align}
for
\begin{align}
	&\|\vstar_{\mathcal{I}_{\widehat{j}}^{c}}\|^2_2 = 1 - p + o(p), \quad \|\beta_{t-1}\|_2 = 1, \quad
	\alpha_{t} = (1 - p + o(p)) \cdot \lambda + O\left(\sqrt{\frac{k + t\log^3 n}{n}}\right),\\
	\text{and}\qquad &\ltwo{\xi}^2 \lesssim (1 - p) \sqrt{\frac{k+t\log^3 n}{n}},
\end{align}
where each $\phi_j \stackrel{\text{i.i.d.}}{\sim} \mathcal{N}(0, \frac{1}{n} I_{|\mathcal{I}^c_{\widehat{j}}|}).$



Now moving on to the second AMP sequence. 
Here, we remind the readers that by construction $\overline{\mathcal{I}}_{\widehat{i}} \subset \mathcal{I}_{\widehat{j}}^{c}$, which implies $\mathcal{I}_{\widehat{j}} \subset \overline{\mathcal{I}}_{\widehat{i}}^{c}.$
Similarly, execution of AMP on $M_{\overline{\mathcal{I}}_{\widehat{i}}^c,\overline{\mathcal{I}}_{\widehat{i}}^c}$ yields the decomposition  
\begin{align}
\label{eqn:decomp-2-sparse}
	\overline{x}_{t}^\ell 
	= \overline{\alpha}_{t} \vstar_\ell + \sum_{j = 1}^{t-1} \overline{\beta}_{t-1}^j \overline{\phi}_{j, \ell} + \overline{\xi}_{t-1, \ell},
	\qquad
	\ell \in \overline{\mathcal{I}}_{\widehat{i}}^{c}, 
\end{align}
\end{subequations}
where the parameters satisfy expressions~\eqref{eqn:finale-prop3}.
Note that here, we take the union bound over $N \times N$ choices of index $\widehat{j} \in N$ and index $\widehat{i} \in N$ (where for each set $\mathcal{I}_j$, we construct $N$ such $\overline{\mathcal{I}}_i \subset
\mathcal{I}_{j}^c$). 


Taking these two decompositions collectively, we can write the output $u_{t}$ (defined in \eqref{eqn:estimate-u}) as
\begin{align*}
	u_t = \alpha_{t} \vstar + \sum_{j = 1}^{t-1}\beta_{t-1}^j \phi_{j} + \widetilde{\xi}_{t-1}.
\end{align*}
Here, $\{\phi_{j}\}$ are elongated to an $n$-dimensional Gaussian with $\phi_j\stackrel{\mathrm{i.i.d.}}{\sim} \mathcal{N}(0,\frac{1}{n}I_n)$
and 
\begin{align*}
\widetilde{\xi}_{t-1, \mathcal{I}_{\widehat{j}}^{c}} = \xi_{t-1, \mathcal{I}_{\widehat{j}}^{c}}, 
\qquad
\widetilde{\xi}_{t-1, \mathcal{I}_{\widehat{j}}} = (\overline{\alpha}_{t} - \alpha_t) \vstar_{\mathcal{I}_{\widehat{j}}} + \sum_{j = 1}^{t-1} \overline{\beta}_{t-1}^j\overline{\phi}_{j, \mathcal{I}_{\widehat{j}}} - \sum_{j = 1}^{t-1} \beta_{t-1}^j\phi_{j, \mathcal{I}_{\widehat{j}}} + \overline{\xi}_{t-1, \mathcal{I}_{\widehat{j}}}.
\end{align*}
Comparing this with~\eqref{eqn:decomp-1-sparse} and \eqref{eqn:decomp-2-sparse} and according to Theorem~\ref{thm:sparse}, one has
\begin{align*}
\|\widetilde{\xi}_{t-1}\|_2 
&\le 
\|\xi_{t-1, \mathcal{I}_{\widehat{j}}^c}\|_2 + \|\widetilde{\xi}_{t-1, \mathcal{I}_{\widehat{j}}}\|_2 \\
%
&\leq (1-p)\sqrt{\frac{k+t\log^3 n}{n}} + |\overline{\alpha}_{t} - \alpha_t| p +
\red{\sqrt{\frac{t\log n}{n}} \cdot \sqrt{np}} + \|\overline{\xi}_{t-1, \overline{\mathcal{I}_{\widehat{i}}}^{c}}\|_2 
\lesssim 
 \frac{\lambda \log^2 n}{k^2} + \sqrt{\frac{k+t\log^3 n}{n}}.
\end{align*}
where the penultimate step uses $\ltwo{\beta_{t-1}} = \ltwo{\overline{\beta}_{t-1}} = 1$ and relation \eqref{eqn:simple-rm}, and the last step uses $p \asymp \frac{\log n}{k}$.
Thus, we complete the proof of inequality~\eqref{eqn:decomp-u}. 
 


